A Learning-Based Approach to Address Complexity-Reliability Tradeoff in OS Decoders

In this paper, we study the tradeoffs between complexity and reliability for decoding large linear block codes. We show that using artificial neural networks to predict the required order of an ordered statistics based decoder helps in reducing the average complexity and hence the latency of the decoder. We numerically validate the approach through Monte Carlo simulations.

==> figures.tex <==

\begin{figure*}
    \centering
    \begin{minipage}{\columnwidth}
        \centering
        \includegraphics[width=1\textwidth]{Figures/TEP_bounded_OS_genmat.128.064.022.pdf} 
        \caption{Comparison of the number of evaluated TEPs (i.e reconfigurations) for $ N=128 $ and $ K = 64 $ (eBCH(128,64,22)), between the bound based baseline when $E_b/N_0$ is known (red), bound based baseline when $E_b/N_0$ is estimated (green), and learning-based classifier NN approach (blue) and  learning-based threshold approach (orange). Reference lines (dashed black) represent the number of evaluated TEPs of the regular OS decoder (orders from 0 to 2).}
        \label{fig:AWGN}
    \end{minipage}\hfill
    \begin{minipage}{\columnwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{CER_errors_bounded_OS_Zgenmat.128.064.022.pdf} % second figure itself
        \caption{Comparison of the code error rates for $ N=128 $ and $ K = 64 $ (eBCH(128,64,22)). Please refer to figure~\ref{fig:AWGN} for the information on color codes.}
        \label{fig:AWGNCER}
    \end{minipage}
\end{figure*}
